ASKIT: Approximate Skeletonization Kernel-Independent Treecode in High Dimensions

We present a fast algorithm for kernel summation problems in high-dimensions. These problems appear in computational physics, numerical approximation, non-parametric statistics, and machine learning. In our context, the sums depend on a kernel function that is a pair potential defined on a dataset of points in a high-dimensional Euclidean space. A direct evaluation of the sum scales quadratically with the number of points. Fast kernel summation methods can reduce this cost to linear complexity, but the constants involved do not scale well with the dimensionality of the dataset. The main algorithmic components of fast kernel summation algorithms are the separation of the kernel sum between near and far field (which is the basis for pruning) and the efficient and accurate approximation of the far field. We introduce novel methods for pruning and approximating the far field. Our far field approximation requires only kernel evaluations and does not use analytic expansions. Pruning is not done using bounding boxes but rather combinatorially using a sparsified nearest-neighbor graph of the input. The time complexity of our algorithm depends linearly on the ambient dimension. The error in the algorithm depends on the low-rank approximability of the far field, which in turn depends on the kernel function and on the intrinsic dimensionality of the distribution of the points. The error of the far field approximation does not depend on the ambient dimension. We present the new algorithm along with experimental results that demonstrate its performance. We report results for Gaussian kernel sums for 100 million points in 64 dimensions, for one million points in 1000 dimensions, and for problems in which the Gaussian kernel has a variable bandwidth. To the best of our knowledge, all of these experiments are impossible or prohibitively expensive with existing fast kernel summation methods.

==> figures.tex <==



%\begin{figure}[tbph]
%        \centering
%        \subfigure[\textbf{The binary tree.}  Points belonging to different leaves have distinct colors.]{\includegraphics[width=0.45\textwidth]{figures/tree.pdf}}
%        \subfigure[\textbf{Skeletonizing a leaf.}  The points to be approximated are marked with triangles. The nearest neighbors are marked with squares, and the randomly sampled points with circles.]{\includegraphics[width=0.45\textwidth]{figures/skeletonize_leaf.pdf}}
%        \subfigure[\textbf{Skeletonizing an internal node.}  The skeletons of the children are marked with triangles. The nearest neighbors are marked with squares, and the randomly sampled points with circles.]{\includegraphics[width=0.45\textwidth]{figures/skeletonize_internal.pdf}}
%        \subfigure[\textbf{Downward pass.}  The target point is marked with a star.  The points marked with squares must be evaluated directly.  All other nodes can be pruned and are approximated by computing the evaluation with their skeleton points (triangles).]{\includegraphics[width=0.45\textwidth]{figures/downward_pass.pdf}}
%\caption{The key features of our algorithm. 
%\label{fig_alg_steps}}
%\end{figure}

We include the following illustrations of the key steps of our
algorithm.  These are intended to assist the reader in understanding
of our method.  There are no additional technical details in this
supplementary material. 
\begin{figure}[tbph]
	\centering
        \includegraphics[width=0.45\textwidth]{figures/detailed_figures/tree.pdf}
        \caption{\textbf{The tree.}  An illustration of our
          median-split binary tree. We split a node by estimating the
          farthest pair of points in it.  We project all points onto
          the line between these points, then split at the median.
          The splitting planes are shown, and points belonging to
          different nodes are shown in different colors.
        \label{fig_tree}}
\end{figure}


\begin{figure}[tbph]
	\centering
        %\subfigure[\textbf{Skeletonize Leaf.} .]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/skeletonize_leaf_1.pdf}}
        \subfigure[A leaf node.\label{subfig_leaf_1}]
        		{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/skeletonize_leaf_2.pdf}}
        \subfigure[The node's nearest neighbors.\label{subfig_leaf_2}]
		{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/skeletonize_leaf_3.pdf}}
        \subfigure[Sampling distant points.\label{subfig_leaf_3}]
		{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/skeletonize_leaf_4.pdf}}
        \subfigure[The resulting skeleton.\label{subfig_leaf_4}]
        {\includegraphics[width=0.45\textwidth]{figures/detailed_figures/skeletonize_leaf_5.pdf}}
	\caption{\textbf{Skeletonizing a leaf.}
    \textbf{Fig.~\ref{subfig_leaf_1}.} We highlight the leaf node to
    be skeletonized. The points to be approximated are shown with
    triangles.  \textbf{Fig.~\ref{subfig_leaf_2}.} We compute the
    union of the lists of nearest neighbors of the points in the leaf,
    and exclude points that belong to the leaf itself.  These points
    are highlighted with squares.  \textbf{Fig.~\ref{subfig_leaf_3}.}
    We sample additional distant points for the skeletonization.
    These points are highlighted with circles. We compute the matrix
    of interactions with rows given by the neighbors and samples
    (squares and circles) and columns given by the points in the leaf
    (triangles).  \textbf{Fig.~\ref{subfig_leaf_4}.} We compute the ID
    of this matrix to obtain the skeleton points, highlighted with
    diamonds. Notice that the node has two more points that are not
    part of the skeleton and will not be used for far-field
    evaluations.  We can now approximate the contribution of the
    points in this node to a distant target point using only the
    interactions with these skeleton points.
	\label{fig_skeletonize_leaf}}
\end{figure}
        

\begin{figure}[tbph]
        \centering
        \subfigure[An internal node. \label{subfig_internal_1}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/skeletonize_internal_1.pdf}}
        \subfigure[Merging the neighbor lists. \label{subfig_internal_2}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/skeletonize_internal_2.pdf}}
        \subfigure[Sampling distant points.\label{subfig_internal_3}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/skeletonize_internal_3.pdf}}
        \subfigure[The resulting skeleton.\label{subfig_internal_4}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/skeletonize_internal_4.pdf}}
\caption{\textbf{Skeletonizing an internal node.}
  \textbf{Fig.~\ref{subfig_leaf_1}.} We skeletonize the highlighted
  internal node. The skeletons of its children are highlighted with
  diamonds.  \textbf{Fig.~\ref{subfig_leaf_2}.} We merge the nearest
  neighbor lists of the children, then exclude all of the points
  belonging to the node to be skeletonized. Finding these points can
  be done in $\bigO(1)$ time using the Morton ids.  These points are
  highlighted with squares.  \textbf{Fig.~\ref{subfig_leaf_3}.} We
  sample additional distant points, highlighted with circles.  We
  compute the matrix of interactions with rows given by the neighbors
  and samples (squares and circles) and columns given by skeletons of
  the child nodes (triangles).  \textbf{Fig.~\ref{subfig_leaf_4}.} We
  compute the ID of this matrix to obtain a skeleton for the parent
  node, which is a subset of the combined skeletons of the children.
\label{fig_skeletonize_internal_node}}
\end{figure}


\begin{figure}[tbph]
	\centering
        %\subfigure[\textbf{Downward Pass.} .]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/downward_pass_1.pdf}}
        \subfigure[Evaluating at a target point (star).\label{subfig_downward_1}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/downward_pass_2.pdf}}
        \subfigure[Pruning the highlighted node.\label{subfig_downward_2}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/downward_pass_3.pdf}}
        \subfigure[Pruning another node.\label{subfig_downward_3}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/downward_pass_4.pdf}}
        \subfigure[Pruning a leaf node.\label{subfig_downward_4}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/downward_pass_5.pdf}}
        \subfigure[Pruning another leaf node.\label{subfig_downward_5}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/downward_pass_6.pdf}}
        %\subfigure[\textbf{Downward Pass.}\label{subfig_downward_6}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/downward_pass_7.pdf}}
        \subfigure[Directly evaluating un-prunable leaves.\label{subfig_downward_6}]{\includegraphics[width=0.45\textwidth]{figures/detailed_figures/downward_pass_8.pdf}}
\caption{\textbf{Evaluating the approximate summation.}
  \textbf{Fig.~\ref{subfig_downward_1}.} We evaluate the potential at
  a target point, highlighted with a star. We show its nearest nearest
  neighbors as well, highlighted with squares.
  \textbf{Fig.~\ref{subfig_downward_2}.} We traverse the tree in a top
  down fashion.  We can prune a node if the node does not contain any
  neighbors of the target point. By pruning we mean evaluating the
  field of the node using the skeleton on the target point and then
  terminating the traversal.  The node highlighted in red satisfies
  our pruning criterion, so we evaluate its contribution
  approximately.  We compute the interactions between the skeleton
  points (diamonds) and the target. We use the skeleton weights for
  these points to compute the effective contribution of the node.
  \textbf{Fig.~\ref{subfig_downward_3}.} We continue traversing the
  tree.  Once again, we have a node that contains no nearest neighbors
  of the target, so we use the skeleton points to compute its
  approximate contribution.  \textbf{Fig.~\ref{subfig_downward_4}.} We
  still use the approximate representation at leaves which satisfy the
  pruning criterion.  \textbf{Fig.~\ref{subfig_downward_5}.} We
  continue the approximate evaluation of all nodes that satisfy the
  pruning criterion.  \textbf{Fig.~\ref{subfig_downward_6}.} The
  leaves highlighted in blue do not satisfy the pruning criterion, so
  we compute their contribution directly.  We evaluate the direct
  interaction between all points in these nodes (highlighted with
  squares) and the target point.
\label{fig_alg_steps}}
\end{figure}




==> laplace_results.tex <==

These are the preliminary experiments for the Laplace kernel in ASKIT.

\begin{table}[htb]
\centering
\begin{tabular}{| l | ll | lll | llll | ll |} \hline
{\bf run}  &  $\boldsymbol{\ppl}$  &  $\boldsymbol{\ns}$  &  {\bf hr}  &  $\boldsymbol{\epsilon}$  &  $\boldsymbol{\epsilon}_\kappa$  &  $\boldsymbol{T}_\kappa$  &  $\boldsymbol{T}$  &  $\boldsymbol{T}_S$  &  $\boldsymbol{T}_E$  &  {\bf near}  &  ${\bf far}$  \\ \hline
-- &  64  &  4  &  99  &  1E+00  &  1E+00  &  8  &  2  &  0  &  1  &  5  &  1  \\ 
-- &  64  &  32  &  99  &  1E+00  &  1E+00  &  8  &  3  &  0  &  3  &  5  &  1  \\ 
-- &  64  &  128  &  99  &  5E-01  &  1E+00  &  8  &  4  &  0  &  3  &  5  &  1  \\ 
-- &  64  &  256  &  99  &  4E-03  &  1E+00  &  8  &  4  &  1  &  3  &  5  &  1  \\ \hline
-- &  256  &  4  &  99  &  1E+00  &  1E+00  &  10  &  2  &  1  &  2  &  1  &  0  \\ 
-- &  256  &  32  &  99  &  1E+00  &  1E+00  &  10  &  3  &  1  &  2  &  1  &  0  \\ 
-- &  256  &  128  &  99  &  4E-01  &  1E+00  &  10  &  3  &  1  &  2  &  1  &  0  \\ 
-- &  256  &  256  &  98  &  4E-03  &  1E+00  &  15  &  4  &  1  &  3  &  1  &  0  \\ \hline
-- &  512  &  4  &  95  &  1E+00  &  1E+00  &  14  &  4  &  1  &  3  &  1  &  0  \\ 
-- &  512  &  32  &  95  &  1E+00  &  1E+00  &  15  &  4  &  1  &  3  &  1  &  0  \\ 
-- &  512  &  128  &  95  &  5E-01  &  1E+00  &  15  &  5  &  1  &  4  &  1  &  0  \\ 
-- &  512  &  256  &  95  &  4E-03  &  1E+00  &  15  &  6  &  1  &  4  &  1  &  0  \\ \hline
\end{tabular}
\caption{\label{table_askit_laplace_2D_100k_normal}
Results for \ASKIT~algorithm on \textbf{Laplace kernel} with \textbf{2D Gaussian data, $N = 10^5$}. 
Legend: "$\boldsymbol{\ppl}$" -- leaf size, "$\boldsymbol{\ns}$" -- rank of ID, "{\bf hr}"  -- hit rate of NN
search, "$\boldsymbol{\epsilon}$" -- Error of \ASKIT~averaged over 1000 direct evals, 
"$\boldsymbol{\epsilon}_\kappa$" -- Error in NN search, "$\boldsymbol{T}_\kappa$" -- time for NN search and
tree building, "$\boldsymbol{T}$" -- total time for \ASKIT~(excluding NN search), 
"$\boldsymbol{T}_S$" -- time to build skeletons, "$\boldsymbol{T}_E$" -- time to evaluate potentials,
"{\bf near}" -- Number of nodes evaluated directly per target, "{\bf far}"
-- number of nodes evaluated approximately per target. All experiments used 
$d + 8$ iterations of neighbor search, number of neighbors equal to $2 \times
m$, number of skeleton targets equal to $s + 20$. All experiments on a single
node of Maverick with 20 OpenMP threads. 
}
\end{table}

\begin{table}[htb]
\centering
\begin{tabular}{| l | ll | lll | llll | ll |} \hline
{\bf run}  &  $\boldsymbol{\ppl}$  &  $\boldsymbol{\ns}$  &  {\bf hr}  &  $\boldsymbol{\epsilon}$  &  $\boldsymbol{\epsilon}_\kappa$  &  $\boldsymbol{T}_\kappa$  &  $\boldsymbol{T}$  &  $\boldsymbol{T}_S$  &  $\boldsymbol{T}_E$  &  {\bf near}  &  ${\bf far}$  \\ \hline
-- &  64  &  4  &  99  &  9E-01  &  1E+00  &  9  &  3  &  0  &  3  &  9  &  2  \\ 
-- &  64  &  32  &  99  &  6E-01  &  1E+00  &  9  &  4  &  0  &  4  &  9  &  2  \\ 
-- &  64  &  128  &  99  &  3E-01  &  1E+00  &  9  &  6  &  0  &  5  &  9  &  2  \\ 
-- &  64  &  256  &  99  &  2E-01  &  1E+00  &  17  &  5  &  1  &  4  &  9  &  2  \\ \hline
-- &  256  &  4  &  97  &  9E-01  &  1E+00  &  10  &  3  &  1  &  3  &  3  &  0  \\ 
-- &  256  &  32  &  97  &  6E-01  &  1E+00  &  11  &  5  &  1  &  4  &  3  &  0  \\ 
-- &  256  &  128  &  97  &  3E-01  &  1E+00  &  11  &  5  &  1  &  4  &  3  &  0  \\ 
-- &  256  &  256  &  97  &  2E-01  &  1E+00  &  11  &  6  &  1  &  4  &  3  &  0  \\ \hline
-- &  512  &  4  &  90  &  8E-01  &  9E-01  &  17  &  6  &  1  &  5  &  1  &  0  \\ 
-- &  512  &  32  &  90  &  5E-01  &  9E-01  &  15  &  6  &  1  &  5  &  1  &  0  \\ 
-- &  512  &  128  &  90  &  3E-01  &  9E-01  &  15  &  7  &  1  &  6  &  1  &  0  \\ 
-- &  512  &  256  &  90  &  2E-01  &  9E-01  &  16  &  8  &  1  &  7  &  1  &  0  \\ \hline
\end{tabular}
\caption{\label{table_askit_laplace_3D_100k_normal}
Results for \ASKIT~algorithm on \textbf{Laplace kernel} with \textbf{3D Gaussian data, $N = 10^5$}. 
Legend: "$\boldsymbol{\ppl}$" -- leaf size, "$\boldsymbol{\ns}$" -- rank of ID, "{\bf hr}"  -- hit rate of NN
search, "$\boldsymbol{\epsilon}$" -- Error of \ASKIT~averaged over 1000 direct evals, 
"$\boldsymbol{\epsilon}_\kappa$" -- Error in NN search, "$\boldsymbol{T}_\kappa$" -- time for NN search and
tree building, "$\boldsymbol{T}$" -- total time for \ASKIT~(excluding NN search), 
"$\boldsymbol{T}_S$" -- time to build skeletons, "$\boldsymbol{T}_E$" -- time to evaluate potentials,
"{\bf near}" -- Number of nodes evaluated directly per target, "{\bf far}"
-- number of nodes evaluated approximately per target. All experiments used 
$d + 8$ iterations of neighbor search, number of neighbors equal to $2 \times
m$, number of skeleton targets equal to $s + 20$. All experiments on a single
node of Maverick with 20 OpenMP threads. 
}
\end{table}

\begin{table}[htb]
\centering
\begin{tabular}{| l | ll | lll | llll | ll |} \hline
{\bf run}  &  $\boldsymbol{\ppl}$  &  $\boldsymbol{\ns}$  &  {\bf hr}  &  $\boldsymbol{\epsilon}$  &  $\boldsymbol{\epsilon}_\kappa$  &  $\boldsymbol{T}_\kappa$  &  $\boldsymbol{T}$  &  $\boldsymbol{T}_S$  &  $\boldsymbol{T}_E$  &  {\bf near}  &  ${\bf far}$  \\ \hline
-- &  64  &  4  &  99  &  9E-01  &  1E+00  &  10  &  5  &  0  &  4  &  15  &  3  \\ 
-- &  64  &  32  &  99  &  8E-01  &  1E+00  &  16  &  7  &  0  &  6  &  15  &  3  \\ 
-- &  64  &  128  &  99  &  5E-01  &  1E+00  &  19  &  10  &  1  &  9  &  15  &  3  \\ 
-- &  64  &  256  &  99  &  4E-01  &  1E+00  &  9  &  8  &  1  &  7  &  15  &  3  \\ \hline
-- &  256  &  4  &  94  &  8E-01  &  9E-01  &  12  &  5  &  1  &  4  &  5  &  1  \\ 
-- &  256  &  32  &  94  &  7E-01  &  9E-01  &  11  &  6  &  1  &  5  &  5  &  1  \\ 
-- &  256  &  128  &  94  &  5E-01  &  9E-01  &  11  &  7  &  1  &  6  &  5  &  1  \\ 
-- &  256  &  256  &  95  &  3E-01  &  9E-01  &  11  &  8  &  1  &  7  &  5  &  1  \\ \hline
-- &  512  &  4  &  88  &  7E-01  &  9E-01  &  17  &  8  &  1  &  7  &  2  &  0  \\ 
-- &  512  &  32  &  88  &  6E-01  &  9E-01  &  17  &  8  &  1  &  7  &  2  &  0  \\ 
-- &  512  &  128  &  88  &  4E-01  &  9E-01  &  18  &  9  &  1  &  8  &  2  &  0  \\ 
-- &  512  &  256  &  88  &  3E-01  &  9E-01  &  17  &  10  &  1  &  9  &  2  &  0  \\ \hline
\end{tabular}
\caption{\label{table_askit_laplace_4D_100k_normal}
Results for \ASKIT~algorithm on \textbf{Laplace kernel} with \textbf{4D Gaussian data, $N = 10^5$}. 
Legend: "$\boldsymbol{\ppl}$" -- leaf size, "$\boldsymbol{\ns}$" -- rank of ID, "{\bf hr}"  -- hit rate of NN
search, "$\boldsymbol{\epsilon}$" -- Error of \ASKIT~averaged over 1000 direct evals, 
"$\boldsymbol{\epsilon}_\kappa$" -- Error in NN search, "$\boldsymbol{T}_\kappa$" -- time for NN search and
tree building, "$\boldsymbol{T}$" -- total time for \ASKIT~(excluding NN search), 
"$\boldsymbol{T}_S$" -- time to build skeletons, "$\boldsymbol{T}_E$" -- time to evaluate potentials,
"{\bf near}" -- Number of nodes evaluated directly per target, "{\bf far}"
-- number of nodes evaluated approximately per target. All experiments used 
$d + 8$ iterations of neighbor search, number of neighbors equal to $2 \times
m$, number of skeleton targets equal to $s + 20$. All experiments on a single
node of Maverick with 20 OpenMP threads. 
}
\end{table}

\begin{table}[htb]
\centering
\begin{tabular}{| l | ll | lll | llll | ll |} \hline
{\bf run}  &  $\boldsymbol{\ppl}$  &  $\boldsymbol{\ns}$  &  {\bf hr}  &  $\boldsymbol{\epsilon}$  &  $\boldsymbol{\epsilon}_\kappa$  &  $\boldsymbol{T}_\kappa$  &  $\boldsymbol{T}$  &  $\boldsymbol{T}_S$  &  $\boldsymbol{T}_E$  &  {\bf near}  &  ${\bf far}$  \\ \hline
-- &  64  &  4  &  98  &  8E-01  &  9E-01  &  10  &  6  &  0  &  6  &  21  &  4  \\ 
-- &  64  &  32  &  98  &  7E-01  &  9E-01  &  10  &  9  &  0  &  9  &  21  &  4  \\ 
-- &  64  &  128  &  98  &  5E-01  &  9E-01  &  11  &  11  &  1  &  11  &  21  &  4  \\ 
-- &  64  &  256  &  98  &  4E-01  &  9E-01  &  10  &  10  &  1  &  10  &  21  &  4  \\ \hline
-- &  256  &  4  &  91  &  6E-01  &  8E-01  &  12  &  6  &  1  &  6  &  7  &  1  \\ 
-- &  256  &  32  &  91  &  6E-01  &  8E-01  &  13  &  7  &  1  &  7  &  7  &  1  \\ 
-- &  256  &  128  &  91  &  4E-01  &  8E-01  &  13  &  9  &  1  &  8  &  7  &  1  \\ 
-- &  256  &  256  &  92  &  3E-01  &  8E-01  &  13  &  10  &  1  &  9  &  7  &  1  \\ \hline
-- &  512  &  4  &  84  &  5E-01  &  8E-01  &  18  &  10  &  1  &  9  &  3  &  0  \\ 
-- &  512  &  32  &  84  &  5E-01  &  8E-01  &  19  &  11  &  1  &  10  &  3  &  0  \\ 
-- &  512  &  128  &  84  &  4E-01  &  8E-01  &  19  &  12  &  1  &  11  &  3  &  0  \\ 
-- &  512  &  256  &  84  &  3E-01  &  8E-01  &  18  &  13  &  1  &  12  &  3  &  0  \\ \hline
\end{tabular}
\caption{\label{table_askit_laplace_5D_100k_normal}
Results for \ASKIT~algorithm on \textbf{Laplace kernel} with \textbf{5D Gaussian data, $N = 10^5$}. 
Legend: "$\boldsymbol{\ppl}$" -- leaf size, "$\boldsymbol{\ns}$" -- rank of ID, "{\bf hr}"  -- hit rate of NN
search, "$\boldsymbol{\epsilon}$" -- Error of \ASKIT~averaged over 1000 direct evals, 
"$\boldsymbol{\epsilon}_\kappa$" -- Error in NN search, "$\boldsymbol{T}_\kappa$" -- time for NN search and
tree building, "$\boldsymbol{T}$" -- total time for \ASKIT~(excluding NN search), 
"$\boldsymbol{T}_S$" -- time to build skeletons, "$\boldsymbol{T}_E$" -- time to evaluate potentials,
"{\bf near}" -- Number of nodes evaluated directly per target, "{\bf far}"
-- number of nodes evaluated approximately per target. All experiments used 
$d + 8$ iterations of neighbor search, number of neighbors equal to $2 \times
m$, number of skeleton targets equal to $s + 20$. All experiments on a single
node of Maverick with 20 OpenMP threads. 
}
\end{table}



\begin{table}[htb]
\centering
\begin{tabular}{| l | lll | lll | llll | ll |} \hline
{\bf run}  &  $\boldsymbol{\ppl}$  &  $\boldsymbol{\ns}$  &  {\bf msl}  &  {\bf hr}  &  $\boldsymbol{\epsilon}$  &  $\boldsymbol{\epsilon}_\kappa$  &  $\boldsymbol{T}_\kappa$  &  $\boldsymbol{T}$  &  $\boldsymbol{T}_S$  &  $\boldsymbol{T}_E$  &  {\bf near}  &  ${\bf far}$  \\ \hline
-- &  256  &  128  &  2  &  96  &  3E-01  &  1E+00  &  10  &  5  &  1  &  4  &  3  &  0  \\ 
-- &  256  &  128  &  3  &  96  &  2E-01  &  1E+00  &  11  &  5  &  1  &  4  &  3  &  1  \\ 
-- &  256  &  128  &  4  &  96  &  2E-01  &  1E+00  &  18  &  6  &  1  &  5  &  3  &  1  \\ 
-- &  256  &  128  &  5  &  96  &  1E-01  &  1E+00  &  13  &  10  &  1  &  9  &  3  &  1  \\ 
-- &  256  &  128  &  6  &  96  &  8E-02  &  1E+00  &  15  &  13  &  1  &  12  &  3  &  2  \\ 
-- &  256  &  128  &  7  &  96  &  4E-02  &  1E+00  &  11  &  23  &  1  &  22  &  3  &  3  \\ 
-- &  256  &  128  &  8  &  96  &  1E-02  &  1E+00  &  10  &  42  &  1  &  41  &  3  &  6  \\ 
-- &  256  &  128  &  9  &  96  &  3E-04  &  1E+00  &  11  &  82  &  1  &  81  &  3  &  11  \\ 
-- &  256  &  128  &  10  &  96  &  5E-16  &  1E+00  &  11  &  57  &  0  &  57  &  100  &  0  \\ \hline
-- &  256  &  256  &  2  &  97  &  2E-01  &  1E+00  &  10  &  5  &  1  &  4  &  3  &  0  \\ 
-- &  256  &  256  &  3  &  97  &  1E-01  &  1E+00  &  10  &  6  &  1  &  5  &  3  &  1  \\ 
-- &  256  &  256  &  4  &  96  &  1E-01  &  1E+00  &  10  &  6  &  1  &  5  &  3  &  1  \\ 
-- &  256  &  256  &  5  &  97  &  6E-02  &  1E+00  &  10  &  8  &  1  &  7  &  3  &  1  \\ 
-- &  256  &  256  &  6  &  96  &  3E-02  &  1E+00  &  10  &  11  &  1  &  9  &  3  &  2  \\ 
-- &  256  &  256  &  7  &  96  &  4E-03  &  1E+00  &  10  &  18  &  1  &  17  &  3  &  3  \\ 
-- &  256  &  256  &  8  &  96  &  2E-05  &  1E+00  &  10  &  29  &  1  &  28  &  3  &  6  \\ 
-- &  256  &  256  &  9  &  97  &  5E-16  &  1E+00  &  11  &  68  &  0  &  68  &  3  &  11  \\ 
-- &  256  &  256  &  10  &  96  &  5E-16  &  1E+00  &  11  &  57  &  0  &  57  &  100  &  0  \\ \hline
-- &  256  &  512  &  2  &  96  &  8E-02  &  1E+00  &  17  &  8  &  2  &  5  &  3  &  0  \\ 
-- &  256  &  512  &  3  &  96  &  6E-02  &  1E+00  &  10  &  8  &  2  &  6  &  3  &  1  \\ 
-- &  256  &  512  &  4  &  96  &  4E-02  &  1E+00  &  18  &  9  &  2  &  7  &  3  &  1  \\ 
-- &  256  &  512  &  5  &  96  &  1E-02  &  1E+00  &  10  &  11  &  2  &  9  &  3  &  1  \\ 
-- &  256  &  512  &  6  &  96  &  3E-04  &  1E+00  &  18  &  16  &  2  &  14  &  3  &  2  \\ 
-- &  256  &  512  &  7  &  96  &  2E-06  &  1E+00  &  10  &  24  &  1  &  23  &  3  &  3  \\ 
-- &  256  &  512  &  8  &  96  &  3E-16  &  1E+00  &  10  &  36  &  0  &  36  &  3  &  6  \\ 
-- &  256  &  512  &  9  &  96  &  5E-16  &  1E+00  &  11  &  69  &  0  &  68  &  3  &  11  \\ 
-- &  256  &  512  &  10  &  96  &  5E-16  &  1E+00  &  10  &  57  &  0  &  57  &  100  &  0  \\ \hline
\end{tabular}
\caption{\label{table_askit_laplace_3D_100k_normal_level1}
Results for \ASKIT~algorithm on \textbf{Laplace kernel} with \textbf{3D Gaussian data, $N = 10^5$. Restricted levels for skeletons}. 
Legend: "$\boldsymbol{\ppl}$" -- leaf size, "$\boldsymbol{\ns}$" -- rank of ID,
"{\bf msl}" -- the minimum skeleton level. No skeletons are computed (and no prunes occur) above this level, "{\bf hr}"  -- hit rate of NN
search, "$\boldsymbol{\epsilon}$" -- Error of \ASKIT~averaged over 1000 direct evals, 
"$\boldsymbol{\epsilon}_\kappa$" -- Error in NN search, "$\boldsymbol{T}_\kappa$" -- time for NN search and
tree building, "$\boldsymbol{T}$" -- total time for \ASKIT~(excluding NN search), 
"$\boldsymbol{T}_S$" -- time to build skeletons, "$\boldsymbol{T}_E$" -- time to evaluate potentials,
"{\bf near}" -- Number of nodes evaluated directly per target, "{\bf far}"
-- number of nodes evaluated approximately per target. All experiments used 
$d + 8$ iterations of neighbor search, number of neighbors equal to $2 \times
m$, number of skeleton targets equal to $s + 20$. All experiments on a single
node of Maverick with 20 OpenMP threads. 
}
\end{table}


\begin{table}[htb]
\centering
\begin{tabular}{| l | lll | lll | llll | ll |} \hline
{\bf run}  &  $\boldsymbol{\ppl}$  &  $\boldsymbol{\ns}$  &  {\bf msl}  &  {\bf hr}  &  $\boldsymbol{\epsilon}$  &  $\boldsymbol{\epsilon}_\kappa$  &  $\boldsymbol{T}_\kappa$  &  $\boldsymbol{T}$  &  $\boldsymbol{T}_S$  &  $\boldsymbol{T}_E$  &  {\bf near}  &  ${\bf far}$  \\ \hline
-- &  512  &  128  &  2  &  91  &  3E-01  &  9E-01  &  23  &  7  &  1  &  6  &  1  &  0  \\ 
-- &  512  &  128  &  3  &  91  &  2E-01  &  9E-01  &  16  &  7  &  1  &  6  &  1  &  0  \\ 
-- &  512  &  128  &  4  &  91  &  2E-01  &  9E-01  &  16  &  7  &  1  &  6  &  1  &  0  \\ 
-- &  512  &  128  &  5  &  91  &  1E-01  &  9E-01  &  16  &  8  &  1  &  7  &  1  &  0  \\ 
-- &  512  &  128  &  6  &  91  &  8E-02  &  9E-01  &  24  &  10  &  1  &  9  &  1  &  1  \\ 
-- &  512  &  128  &  7  &  91  &  4E-02  &  9E-01  &  16  &  17  &  1  &  16  &  1  &  2  \\ 
-- &  512  &  128  &  8  &  90  &  1E-02  &  9E-01  &  16  &  37  &  1  &  36  &  1  &  3  \\ 
-- &  512  &  128  &  9  &  91  &  4E-16  &  9E-01  &  15  &  45  &  0  &  45  &  25  &  0  \\ 
-- &  512  &  128  &  10  &  91  &  4E-16  &  9E-01  &  16  &  43  &  0  &  43  &  25  &  0  \\ \hline
-- &  512  &  256  &  2  &  90  &  1E-01  &  9E-01  &  19  &  8  &  1  &  6  &  1  &  0  \\ 
-- &  512  &  256  &  3  &  90  &  1E-01  &  9E-01  &  15  &  8  &  1  &  6  &  1  &  0  \\ 
-- &  512  &  256  &  4  &  90  &  1E-01  &  9E-01  &  18  &  8  &  1  &  7  &  1  &  0  \\ 
-- &  512  &  256  &  5  &  90  &  6E-02  &  9E-01  &  16  &  9  &  1  &  8  &  1  &  0  \\ 
-- &  512  &  256  &  6  &  90  &  3E-02  &  9E-01  &  15  &  12  &  1  &  11  &  1  &  1  \\ 
-- &  512  &  256  &  7  &  90  &  4E-03  &  9E-01  &  15  &  18  &  1  &  17  &  1  &  2  \\ 
-- &  512  &  256  &  8  &  90  &  2E-05  &  9E-01  &  16  &  30  &  1  &  29  &  1  &  3  \\ 
-- &  512  &  256  &  9  &  90  &  3E-16  &  9E-01  &  16  &  46  &  0  &  46  &  25  &  0  \\ 
-- &  512  &  256  &  10  &  90  &  3E-16  &  9E-01  &  16  &  46  &  0  &  46  &  25  &  0  \\ \hline
-- &  512  &  512  &  2  &  90  &  8E-02  &  9E-01  &  15  &  10  &  3  &  7  &  1  &  0  \\ 
-- &  512  &  512  &  3  &  90  &  6E-02  &  9E-01  &  16  &  10  &  3  &  7  &  1  &  0  \\ 
-- &  512  &  512  &  4  &  90  &  5E-02  &  9E-01  &  15  &  11  &  3  &  9  &  1  &  0  \\ 
-- &  512  &  512  &  5  &  90  &  2E-02  &  9E-01  &  15  &  13  &  2  &  11  &  1  &  1  \\ 
-- &  512  &  512  &  6  &  90  &  3E-04  &  9E-01  &  15  &  17  &  2  &  15  &  1  &  1  \\ 
-- &  512  &  512  &  7  &  90  &  1E-06  &  9E-01  &  16  &  26  &  2  &  25  &  1  &  2  \\ 
-- &  512  &  512  &  8  &  90  &  3E-16  &  9E-01  &  16  &  38  &  1  &  37  &  1  &  3  \\ 
-- &  512  &  512  &  9  &  90  &  3E-16  &  9E-01  &  15  &  42  &  0  &  42  &  25  &  0  \\ 
-- &  512  &  512  &  10  &  90  &  3E-16  &  9E-01  &  15  &  46  &  0  &  46  &  25  &  0  \\ \hline
\end{tabular}
\caption{\label{table_askit_laplace_3D_100k_normal_level2}
Results for \ASKIT~algorithm on \textbf{Laplace kernel} with \textbf{3D Gaussian data, $N = 10^5$. Restricted levels for skeletons}. 
Legend: "$\boldsymbol{\ppl}$" -- leaf size, "$\boldsymbol{\ns}$" -- rank of ID,
"{\bf msl}" -- the minimum skeleton level. No skeletons are computed (and no prunes occur) above this level, "{\bf hr}"  -- hit rate of NN
search, "$\boldsymbol{\epsilon}$" -- Error of \ASKIT~averaged over 1000 direct evals, 
"$\boldsymbol{\epsilon}_\kappa$" -- Error in NN search, "$\boldsymbol{T}_\kappa$" -- time for NN search and
tree building, "$\boldsymbol{T}$" -- total time for \ASKIT~(excluding NN search), 
"$\boldsymbol{T}_S$" -- time to build skeletons, "$\boldsymbol{T}_E$" -- time to evaluate potentials,
"{\bf near}" -- Number of nodes evaluated directly per target, "{\bf far}"
-- number of nodes evaluated approximately per target. All experiments used 
$d + 8$ iterations of neighbor search, number of neighbors equal to $2 \times
m$, number of skeleton targets equal to $s + 20$. All experiments on a single
node of Maverick with 20 OpenMP threads. 
}
\end{table}




\begin{table}[htb]
\centering
\begin{tabular}{| l | lll | lll | llll | ll |} \hline
{\bf run}  &  $\boldsymbol{\ppl}$  &  $\boldsymbol{\ns}$  &  {\bf msl}  &  {\bf hr}  &  $\boldsymbol{\epsilon}$  &  $\boldsymbol{\epsilon}_\kappa$  &  $\boldsymbol{T}_\kappa$  &  $\boldsymbol{T}$  &  $\boldsymbol{T}_S$  &  $\boldsymbol{T}_E$  &  {\bf near}  &  ${\bf far}$  \\ \hline
-- &  256  &  128  &  2  &  91  &  4E-01  &  8E-01  &  14  &  9  &  1  &  8  &  7  &  1  \\ 
-- &  256  &  128  &  3  &  91  &  4E-01  &  8E-01  &  12  &  9  &  1  &  8  &  7  &  1  \\ 
-- &  256  &  128  &  4  &  91  &  4E-01  &  8E-01  &  12  &  10  &  1  &  9  &  7  &  1  \\ 
-- &  256  &  128  &  5  &  91  &  4E-01  &  8E-01  &  12  &  11  &  1  &  11  &  7  &  1  \\ 
-- &  256  &  128  &  6  &  92  &  3E-01  &  8E-01  &  12  &  15  &  1  &  14  &  7  &  2  \\ 
-- &  256  &  128  &  7  &  91  &  2E-01  &  8E-01  &  21  &  24  &  1  &  23  &  7  &  3  \\ 
-- &  256  &  128  &  8  &  91  &  1E-01  &  8E-01  &  12  &  42  &  1  &  42  &  7  &  6  \\ 
-- &  256  &  128  &  9  &  91  &  4E-02  &  8E-01  &  12  &  79  &  1  &  78  &  7  &  11  \\ 
-- &  256  &  128  &  10  &  92  &  5E-16  &  8E-01  &  13  &  57  &  0  &  57  &  100  &  0  \\ \hline
-- &  256  &  256  &  2  &  91  &  3E-01  &  8E-01  &  12  &  10  &  1  &  9  &  7  &  1  \\ 
-- &  256  &  256  &  3  &  91  &  3E-01  &  8E-01  &  17  &  10  &  1  &  9  &  7  &  1  \\ 
-- &  256  &  256  &  4  &  91  &  3E-01  &  8E-01  &  13  &  11  &  1  &  10  &  7  &  1  \\ 
-- &  256  &  256  &  5  &  91  &  2E-01  &  8E-01  &  12  &  12  &  1  &  10  &  7  &  1  \\ 
-- &  256  &  256  &  6  &  91  &  2E-01  &  8E-01  &  22  &  14  &  1  &  13  &  7  &  2  \\ 
-- &  256  &  256  &  7  &  91  &  1E-01  &  8E-01  &  13  &  19  &  1  &  18  &  7  &  3  \\ 
-- &  256  &  256  &  8  &  91  &  2E-02  &  8E-01  &  20  &  32  &  1  &  31  &  7  &  6  \\ 
-- &  256  &  256  &  9  &  91  &  5E-16  &  8E-01  &  12  &  61  &  0  &  61  &  7  &  11  \\ 
-- &  256  &  256  &  10  &  91  &  5E-16  &  8E-01  &  21  &  57  &  0  &  57  &  100  &  0  \\ \hline
-- &  256  &  512  &  2  &  91  &  2E-01  &  8E-01  &  13  &  13  &  2  &  11  &  7  &  1  \\ 
-- &  256  &  512  &  3  &  91  &  2E-01  &  8E-01  &  13  &  13  &  2  &  11  &  7  &  1  \\ 
-- &  256  &  512  &  4  &  91  &  2E-01  &  8E-01  &  14  &  14  &  2  &  11  &  7  &  1  \\ 
-- &  256  &  512  &  5  &  91  &  1E-01  &  8E-01  &  18  &  15  &  2  &  13  &  7  &  1  \\ 
-- &  256  &  512  &  6  &  91  &  7E-02  &  8E-01  &  12  &  19  &  2  &  17  &  7  &  2  \\ 
-- &  256  &  512  &  7  &  91  &  7E-03  &  8E-01  &  14  &  27  &  1  &  26  &  7  &  3  \\ 
-- &  256  &  512  &  8  &  91  &  4E-16  &  8E-01  &  13  &  39  &  0  &  38  &  7  &  6  \\ 
-- &  256  &  512  &  9  &  91  &  5E-16  &  8E-01  &  22  &  71  &  0  &  71  &  7  &  11  \\ 
-- &  256  &  512  &  10  &  91  &  5E-16  &  8E-01  &  13  &  53  &  0  &  53  &  100  &  0  \\ \hline
-- &  256  &  1024  &  2  &  92  &  1E-01  &  9E-01  &  12  &  26  &  13  &  13  &  7  &  1  \\ 
-- &  256  &  1024  &  3  &  92  &  1E-01  &  8E-01  &  21  &  28  &  12  &  16  &  7  &  1  \\ 
-- &  256  &  1024  &  4  &  92  &  8E-02  &  9E-01  &  12  &  27  &  11  &  16  &  7  &  1  \\ 
-- &  256  &  1024  &  5  &  92  &  4E-02  &  8E-01  &  17  &  28  &  9  &  18  &  7  &  1  \\ 
-- &  256  &  1024  &  6  &  92  &  1E-03  &  8E-01  &  13  &  30  &  5  &  25  &  7  &  2  \\ 
-- &  256  &  1024  &  7  &  92  &  3E-16  &  9E-01  &  12  &  35  &  0  &  35  &  7  &  3  \\ 
-- &  256  &  1024  &  8  &  92  &  4E-16  &  9E-01  &  14  &  40  &  0  &  40  &  7  &  6  \\ 
-- &  256  &  1024  &  9  &  92  &  5E-16  &  9E-01  &  12  &  64  &  0  &  64  &  7  &  11  \\ \hline
\end{tabular}
\caption{\label{table_askit_laplace_5D_100k_normal_level1}
Results for \ASKIT~algorithm on \textbf{Laplace kernel} with \textbf{5D Gaussian data, $N = 10^5$. Restricted levels for skeletons}. 
Legend: "$\boldsymbol{\ppl}$" -- leaf size, "$\boldsymbol{\ns}$" -- rank of ID,
"{\bf msl}" -- the minimum skeleton level. No skeletons are computed (and no prunes occur) above this level, "{\bf hr}"  -- hit rate of NN
search, "$\boldsymbol{\epsilon}$" -- Error of \ASKIT~averaged over 1000 direct evals, 
"$\boldsymbol{\epsilon}_\kappa$" -- Error in NN search, "$\boldsymbol{T}_\kappa$" -- time for NN search and
tree building, "$\boldsymbol{T}$" -- total time for \ASKIT~(excluding NN search), 
"$\boldsymbol{T}_S$" -- time to build skeletons, "$\boldsymbol{T}_E$" -- time to evaluate potentials,
"{\bf near}" -- Number of nodes evaluated directly per target, "{\bf far}"
-- number of nodes evaluated approximately per target. All experiments used 
$d + 8$ iterations of neighbor search, number of neighbors equal to $2 \times
m$, number of skeleton targets equal to $s + 20$. All experiments on a single
node of Maverick with 20 OpenMP threads. 
}
\end{table}

\begin{table}[htb]
\centering
\begin{tabular}{| l | lll | lll | llll | ll |} \hline
{\bf run}  &  $\boldsymbol{\ppl}$  &  $\boldsymbol{\ns}$  &  {\bf msl}  &  {\bf hr}  &  $\boldsymbol{\epsilon}$  &  $\boldsymbol{\epsilon}_\kappa$  &  $\boldsymbol{T}_\kappa$  &  $\boldsymbol{T}$  &  $\boldsymbol{T}_S$  &  $\boldsymbol{T}_E$  &  {\bf near}  &  ${\bf far}$  \\ \hline
-- &  512  &  128  &  2  &  84  &  4E-01  &  8E-01  &  18  &  12  &  1  &  11  &  3  &  0  \\ 
-- &  512  &  128  &  3  &  85  &  3E-01  &  8E-01  &  19  &  12  &  1  &  11  &  3  &  0  \\ 
-- &  512  &  128  &  4  &  84  &  3E-01  &  8E-01  &  18  &  12  &  1  &  11  &  3  &  0  \\ 
-- &  512  &  128  &  5  &  85  &  3E-01  &  8E-01  &  18  &  13  &  1  &  12  &  3  &  1  \\ 
-- &  512  &  128  &  6  &  84  &  3E-01  &  8E-01  &  20  &  14  &  1  &  13  &  3  &  1  \\ 
-- &  512  &  128  &  7  &  84  &  2E-01  &  8E-01  &  18  &  18  &  1  &  17  &  3  &  1  \\ 
-- &  512  &  128  &  8  &  84  &  1E-01  &  8E-01  &  19  &  29  &  1  &  28  &  3  &  3  \\ 
-- &  512  &  128  &  9  &  84  &  3E-16  &  8E-01  &  19  &  46  &  0  &  46  &  25  &  0  \\ 
-- &  512  &  128  &  10  &  85  &  3E-16  &  8E-01  &  18  &  46  &  0  &  46  &  25  &  0  \\ \hline
-- &  512  &  256  &  2  &  84  &  3E-01  &  8E-01  &  19  &  13  &  1  &  12  &  3  &  0  \\ 
-- &  512  &  256  &  3  &  84  &  3E-01  &  8E-01  &  18  &  13  &  1  &  12  &  3  &  0  \\ 
-- &  512  &  256  &  4  &  84  &  2E-01  &  8E-01  &  18  &  14  &  1  &  12  &  3  &  0  \\ 
-- &  512  &  256  &  5  &  84  &  2E-01  &  8E-01  &  18  &  15  &  1  &  14  &  3  &  1  \\ 
-- &  512  &  256  &  6  &  84  &  1E-01  &  8E-01  &  18  &  17  &  1  &  15  &  3  &  1  \\ 
-- &  512  &  256  &  7  &  84  &  8E-02  &  8E-01  &  19  &  22  &  1  &  20  &  3  &  1  \\ 
-- &  512  &  256  &  8  &  84  &  2E-02  &  8E-01  &  18  &  33  &  1  &  32  &  3  &  3  \\ 
-- &  512  &  256  &  9  &  84  &  4E-16  &  8E-01  &  18  &  46  &  0  &  46  &  25  &  0  \\ 
-- &  512  &  256  &  10  &  84  &  4E-16  &  8E-01  &  18  &  46  &  0  &  46  &  25  &  0  \\ \hline
-- &  512  &  512  &  2  &  83  &  2E-01  &  8E-01  &  27  &  17  &  3  &  14  &  3  &  0  \\ 
-- &  512  &  512  &  3  &  83  &  2E-01  &  8E-01  &  18  &  17  &  3  &  14  &  3  &  0  \\ 
-- &  512  &  512  &  4  &  83  &  1E-01  &  8E-01  &  19  &  17  &  3  &  14  &  3  &  0  \\ 
-- &  512  &  512  &  5  &  84  &  1E-01  &  8E-01  &  18  &  18  &  2  &  16  &  3  &  1  \\ 
-- &  512  &  512  &  6  &  83  &  6E-02  &  8E-01  &  22  &  22  &  2  &  20  &  3  &  1  \\ 
-- &  512  &  512  &  7  &  84  &  5E-03  &  8E-01  &  20  &  29  &  2  &  28  &  3  &  1  \\ 
-- &  512  &  512  &  8  &  84  &  4E-16  &  8E-01  &  18  &  40  &  1  &  39  &  3  &  3  \\ 
-- &  512  &  512  &  9  &  83  &  4E-16  &  8E-01  &  18  &  46  &  0  &  46  &  25  &  0  \\ 
-- &  512  &  512  &  10  &  83  &  4E-16  &  8E-01  &  18  &  46  &  0  &  46  &  25  &  0  \\ \hline
-- &  512  &  1024  &  2  &  84  &  1E-01  &  8E-01  &  19  &  29  &  13  &  16  &  3  &  0  \\ 
-- &  512  &  1024  &  3  &  84  &  9E-02  &  8E-01  &  18  &  54  &  12  &  42  &  3  &  0  \\ 
-- &  512  &  1024  &  4  &  84  &  7E-02  &  8E-01  &  18  &  29  &  11  &  18  &  3  &  0  \\ 
-- &  512  &  1024  &  5  &  84  &  3E-02  &  8E-01  &  18  &  30  &  9  &  21  &  3  &  1  \\ 
-- &  512  &  1024  &  6  &  84  &  9E-04  &  8E-01  &  18  &  33  &  6  &  27  &  3  &  1  \\ 
-- &  512  &  1024  &  7  &  84  &  3E-16  &  8E-01  &  19  &  36  &  1  &  36  &  3  &  1  \\ 
-- &  512  &  1024  &  8  &  84  &  4E-16  &  8E-01  &  19  &  51  &  1  &  50  &  3  &  3  \\ 
-- &  512  &  1024  &  9  &  84  &  4E-16  &  8E-01  &  18  &  46  &  0  &  46  &  25  &  0  \\ 
-- &  512  &  1024  &  10  &  84  &  4E-16  &  8E-01  &  23  &  47  &  0  &  47  &  25  &  0  \\ \hline
\end{tabular}
\caption{\label{table_askit_laplace_5D_100k_normal_level2}
Results for \ASKIT~algorithm on \textbf{Laplace kernel} with \textbf{5D Gaussian data, $N = 10^5$. Restricted levels for skeletons}. 
Legend: "$\boldsymbol{\ppl}$" -- leaf size, "$\boldsymbol{\ns}$" -- rank of ID,
"{\bf msl}" -- the minimum skeleton level. No skeletons are computed (and no prunes occur) above this level, "{\bf hr}"  -- hit rate of NN
search, "$\boldsymbol{\epsilon}$" -- Error of \ASKIT~averaged over 1000 direct evals, 
"$\boldsymbol{\epsilon}_\kappa$" -- Error in NN search, "$\boldsymbol{T}_\kappa$" -- time for NN search and
tree building, "$\boldsymbol{T}$" -- total time for \ASKIT~(excluding NN search), 
"$\boldsymbol{T}_S$" -- time to build skeletons, "$\boldsymbol{T}_E$" -- time to evaluate potentials,
"{\bf near}" -- Number of nodes evaluated directly per target, "{\bf far}"
-- number of nodes evaluated approximately per target. All experiments used 
$d + 8$ iterations of neighbor search, number of neighbors equal to $2 \times
m$, number of skeleton targets equal to $s + 20$. All experiments on a single
node of Maverick with 20 OpenMP threads. 
}
\end{table}



==> tables.tex <==
\begin{table}[htp!]
%\small
\begin{center}
\begin{tabular}{@{}l| l l l| l g l l g r g l l@{}}
\hline
&\multicolumn{3}{c|}{\em parameters}&\multicolumn{3}{c}{\em
    errors}&\multicolumn{4}{c}{\em timings (secs)}&\multicolumn{2}{c}{\em pruning}\\\cline{8-11}
%\cmidrule{2-4}  \cmidrule{5-7} \cmidrule{8-11}  \cmidrule{12-13}
\rowcolor{gray!00}
{\bf run}& $\boldsymbol{\ppl}$& $\boldsymbol{\ns}$&
$\boldsymbol{h}$&{\bf hr}& $\boldsymbol{\epsilon}$&
      $\boldsymbol{\epsilon}_\kappa$& $\boldsymbol{T}_\kappa$&
$\boldsymbol{T}$& $\boldsymbol{T}_S$& $\boldsymbol{T}_E$&{\bf near}& ${\bf far}$\\ 
\hline
&\multicolumn{12}{l}{\em\color{gray!75} 4D Normal distribution,
  $N=100,000$, \quad $T_{\mathrm{direct}}=16$ secs}\\ 
1 &  64&   4& 0.21& 97& 5E-02& 3E-01& 5     & 5     & 1     & 4     & 15\%& 3 \%\\ 
2 &  64&  32& 0.21& 97& 1E-02& 3E-01& 5    & 7     & <1     & 6     & 15\%& 3 \%\\ 
3 & 256& 128& 0.21& 87& 2E-03& 8E-02& 7     & 8     & 1     & 7     & 5 \%& 1 \%\\ 
\hdashline[0.5pt/2pt]
4 &  64&   4& 1.00& 97& 7E-01& 1E+00& 5     & 4     & <1     & 4     & 15\%& 3 \%\\ 
5&  64&  32& 1.00& 97& 6E-02& 1E+00& 5     & 7     & <1     & 6     & 15\%& 3 \%\\ 
6& 256& 128& 1.00& 88& 3E-03& 9E-01& 7    & 8     & 1     & 7     & 5 \%& 1 \%\\ 
\hdashline[0.5pt/2pt]
7&  64&   4& 5.00& 97& 8E-01& 1E+00& 5     & 5     & <1     & 4     & 15\%& 3 \%\\ 
8&  64&  32& 5.00& 97& 1E-04& 1E+00& 5     & 7     & <1     & 6     & 15\%& 3 \%\\ 
9& 256& 128& 5.00& 88& 4E-08& 1E+00& 7     & 8     & 1     & 7     & 5 \%& 1 \%\\ 
\hline
&\multicolumn{12}{l}{\em\color{gray!75} 4D Normal distribution, $N=1,000,000$, \quad $T_{\mathrm{direct}}=1591$ secs}\\ 
10&  64&   4& 0.16& 95& 1E-01& 5E-01& 56    & 37    & 1     & 36    & 14\%& 3 \%\\ 
11 &  64&  32& 0.16& 95& 3E-02& 5E-01& 54    & 71    & 2     & 69    & 14\%& 3 \%\\ 
12 & 256&  32& 0.16& 84& 7E-03& 3E-01& 60    & 81    & 3     & 78    & 5 \%& 1 \%\\ 
&\multicolumn{12}{l}{\em\color{gray!55} Inexact neighbor information}\\ 
13 &  64&   4& 0.16& 26& 3E-01& 8E-01& 31    & 63    & 2     & 61    & 25\%& 4 \%\\ 
14 &  64&  32& 0.16& 26& 5E-02& 8E-01& 31    & 119   & 3     & 117   & 25\%& 4 \%\\ 
15 &  64& 128& 0.16& 27& 3E-02& 8E-01& 31    & 262   & 4     & 257   & 25\%& 4 \%\\ 
\hline
&\multicolumn{12}{l}{\em\color{gray!75} 16D Normal distribution, $N=1,000,000$, \quad $T_{\mathrm{direct}}=1630$ secs}\\ 
16  &  64&  32& 0.45& 35& 1E-03& 3E-03& 57    & 573   & 6     & 568   & 83\%& 23\%\\ 
17 &  64& 128& 0.45& 34& 7E-04& 4E-03& 57    & 725   & 7     & 717   & 83\%& 23\%\\ 
18 & 256& 128& 0.45& 26& 1E-04& 2E-03& 63    & 997   & 10    & 987   & 55\%& 8 \%\\ 
\hdashline[0.5pt/2pt]
19  &  64&  32& 1.76& 35& 7E-02& 1E+00& 57    & 564   & 6     & 559   & 83\%& 23\%\\ 
20 &  64& 128& 1.76& 35& 5E-02& 1E+00& 57    & 729   & 7     & 723   & 83\%& 23\%\\ 
21 & 256& 128& 1.76& 25& 2E-02& 1E+00& 63    & 1011  & 11    & 1000  & 55\%& 8 \%\\ 
\hline
&\multicolumn{12}{l}{\em\color{gray!75} 64D Normal distribution, $N=1,000,000$, \quad $T_{\mathrm{direct}}=1829$ secs}\\ 
22 &  64& 128& 0.75&  8& 3E-15& 3E-15& 63    & 984   & 10    & 974   & 99\%& 40\%\\ 
23 &  64& 128& 2.62&  8& 2E-01& 1E+00& 63    & 985   & 11    & 975   & 99\%& 40\%\\ 
24 &  64& 128& 4.98&  8& 8E-03& 1E+00& 63    & 991   & 10    & 981   & 99\%& 40\%\\ 
\hline
&\multicolumn{12}{l}{\em\color{gray!75}4D Normal distribution, variable $h$, $N=1,000,000$, \quad $T_{\mathrm{direct}}=1622$ secs}\\ 
25 &  64&  32& 1.00& 95& 3E-02& 1E+00& 55    & 145   & 2     & 143   & 14\%& 3 \%\\ 
26 &  64&  32& 5.00& 95& 4E-06& 1E+00& 57    & 144   & 2     & 142   & 14\%& 3 \%\\ 
\hline
&\multicolumn{12}{l}{\em\color{gray!75} 1000D (4d-intrinsic), $N=1,000,000$, \quad $T_{\mathrm{direct}}=7315$ secs}\\ 
27 &  64&  32& 0.75& 99& 6E-02& 1E+00& 204   & 393   & 11    & 382   & 14\%& 3 \%\\ 
28 &  64&  32& 3.75& 99& 2E-06& 1E+00& 195   & 391   & 10    & 381   & 14\%& 3 \%\\ 
\hline
&\multicolumn{12}{l}{\em\color{gray!75} 18D (UCI SUSY), $N=5,000,000$, \quad $T_{\mathrm{direct}}=41,000$ secs}\\ 
30 &  64& 128& 0.40& 91& 1E-01& 7E-01& 709   & 1510  & 32    & 1478  & 43\%& 9 \%\\ 
31 &  64& 128& 1.00& 90& 7E-02& 1E+00& 567   & 1530  & 33    & 1497  & 43\%& 9 \%\\ 
32 &  64& 128& 5.00& 90& 1E-03& 1E+00& 577   & 1566  & 33    & 1533  & 43\%& 9 \%\\ 
\hline
&\multicolumn{12}{l}{\em\color{gray!75} MPI-parallel 128D (4d-intrinsic),
  $N=5,000,000$, \quad $T_{\mathrm{direct}}=280,000$ secs}\\ 
33 &  64& 128& 0.50& 100& 1E-03& 1E+00& 233   & 1339  & 12    & 1158  & 17\%& 9\%\\ 
34 &  64& 128& 0.50& 100& 1E-03& 1E+00& 43    & 170   & 1     & 144 & 17\%& 9\%\\ 
\hline
&\multicolumn{12}{l}{\em\color{gray!75} MPI-parallel 64D
  (4d-intrinsic) 512 nodes, (8,192 cores) $N=100,000,000$ }\\ 
35 &  64& 128& 0.37& 99& 1E-02& 1E+00& 137   & 1305  & 6     & 880   & 16\%& 19\%\\ 
\end{tabular}
\end{center}
\caption{Performance of \ASKIT{}:Here "$\boldsymbol{\ppl}$" is points
  per leaf, "$\boldsymbol{\ns}$" is number of skeleton points,
  "$\boldsymbol{h}$" the kernel bandwidth, "{\bf hr}" is the
  estimated percentage of correct neighbors. The relative error
  "$\boldsymbol{\epsilon}$" is estimated by direct
  evaluation on 10K randomly selected points;
  "$\boldsymbol{\epsilon}_\kappa$" is the error if we only use the
  near field. We report several timings: "$\boldsymbol{T}_\kappa$" is
  the time to construct the nearest neighbor lists, "$\boldsymbol{T}$"
  is the overall time of \ASKIT," $\boldsymbol{T}_S$" is
  skeletonization time, "$\boldsymbol{T}_E$" is evaluation time. To
  illustrate~\eqref{e:time}, we report the number of tree nodes
  visited per point during evaluation. "{\bf near}" is the average
  number of leaves visited as a percentage of the worst case $\kappa$;
  "{\bf far}" the number of nodes whose skeleton was used to evaluate
  the far field as a percentage of the worst case $\kappa
  \log(N/\ppl)$.  Also "$\boldsymbol{T}_{\mathrm{dir}}$" is the
  estimated time for a direct $N^2$ evaluation. All times are in
  seconds. We highlight the error, the treecode time, and the
  evaluation time. "{\bf run}" indexes the experiments.  The two last
  runs (33-34) are done using 16 and 256  nodes respectively
  and the MPI library~\cite{mpi96}. }
\label{t:results}
\end{table}


